Consistent Estimation in General Sublinear Preferential Attachment Trees

We propose an empirical estimator of the preferential attachment function $f$ in the setting of general preferential attachment trees. Using a supercritical continuous-time branching process framework, we prove the almost sure consistency of the proposed estimator. We perform simulations to study the empirical properties of our estimators.

==> aad.tex <==
\catcode`\@=11 % allows @ to be used in control sequences in this format file


% \newtheorem{theorem}{Theorem}%[section]
% \newtheorem{lemma}{Lemma}%[section]
% \newtheorem{definition}{Definition}%[section]
% \newtheorem{corollary}{Corollary}%[section]
% \newtheorem{proposition}{Proposition}%[section]
% \newtheorem{example}{Example}%[section]
% \newcommand{\prf}{\begin{proof}{Proof}}
%\renewcommand{\endproof}{\end{proof}}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}[theorem]{Lemma}%[section]
\newtheorem{definition}[theorem]{Definition}%[section]
\newtheorem{corollary}[theorem]{Corollary}%[section]
\newtheorem{proposition}[theorem]{Proposition}%[section]
\newtheorem{example}[theorem]{Example}%[section]


\def\itemi{\item{(i)}}
\def\itemii{\item{(ii)}}
\def\itemiii{\item{(iii)}}
\def\itemiv{\item{(iv)}}
\def\itemv{\item{(v)}}
\def\itemvi{\item{(vi)}}


% Abbreviations
\def\A{{\cal A}} \def\a{{\alpha}}
\def\B{{\cal B}} \def\b{{\beta}}                        \def\BB{\mathbb{B}} \def\bB{{\bf B}}
\def\C{{\cal C}}                                        \def\CC{\mathbb{C}}
\def\D{{\cal D}} \def\d{{\delta}}     \def\gD{{\Delta}} \def\DD{\mathbb{D}}
                 \def\e{{\varepsilon}}                  \def\EE{\mathbb{E}} \def\bE{{\bf E}}
\def\F{{\cal F}} \def\f{{\phi}}                         \def\FF{\mathbb{F}}
\def\G{{\cal G}} \def\g{{\gamma}}                       \def\GG{\mathbb{G}}                           
\def\H{{\cal H}} \def\h{{\eta}}                         \def\HH{\mathbb{H}} \def\bH{{\bf H}}
\def\I{{\cal I}}                                        \def\II{\mathbb{I}} 
\def\J{{\cal J}}                                        \def\JJ{\mathbb{J}}              
\def\K{{\cal K}} \def\k{{\kappa}}                       \def\KK{\mathbb{K}}                              
\def\L{{\cal L}} \def\l{{\lambda}}    \def\gL{{\Lambda}}\def\LL{\mathbb{L}} \def\bL{{\bf L}}
\def\M{{\cal M}} \def\m{{\mu}}                          \def\MM{\mathbb{M}}
                 \def\n{{\nu}}                          \def\NN{\mathbb{N}}                              
\def\O{{\Omega}} \def\o{{\omega}}
\def\P{{\cal P}} \def\p{{\pi}}                          \def\PP{\mathbb{P}}
\def\Q{{\cal Q}} \def\q{{\theta}}                       \def\QQ{\mathbb{Q}}
\def\R{{\cal R}} \def\r{{\rho}}				\def\RR{\mathbb{R}}
                 \def\s{{\sigma}}     \def\S{{\Sigma}}  \def\SS{\mathbb{S}}
                 \def\t{{\tau}}       \def\T{{\Theta}}
\def\U{{\cal U}}					\def\UU{\mathbb{U}}
							\def\VV{\mathbb{V}}
\def\W{{\cal W}}                                        \def\WW{\mathbb{W}}
\def\X{{\cal X}} \def\x{{\xi}}				\def\XX{\mathbb{X}} \def\bX{{\bf X}}
\def\Y{{\cal Y}}					\def\YY{\mathbb{Y}} \def\bY{{\bf Y}}
\def\Z{{\cal Z}} \def\z{{\zeta}}                        \def\ZZ{\mathbb{Z}}


\def\sumin{{\sum_{i=1}^n}}
\def\sumjn{{\sum_{j=1}^n}}
\def\sumim{{\sum_{i=1}^m}}
\def\sumjm{{\sum_{j=1}^m}}
\def\sumik{{\sum_{i=1}^k}}
\def\sumjk{{\sum_{j=1}^k}}
\def\tsum{{\textstyle\sum\limits}}
\def\prodjn{{\prod_{j=1}^n}}
\def\prodin{{\prod_{i=1}^n}}
\def\prodim{{\prod_{i=1}^m}}
\def\prodjm{{\prod_{j=1}^m}}
\def\prodik{{\prod_{i=1}^k}}
\def\tprodik{\textstyle\prod_{i=1}^k\limits}
\def\tprod{{\textstyle\prod\limits}}
\def\prodm{\otimes} 
\def\prodmjn{{\bigotimes_{j=1}^n}}
\def\prodmin{{\bigotimes_{i=1}^n}}
\def\tprodmin{{\textstyle\bigotimes_{i=1}^n\limits}}
\def\tprodmjn{{\textstyle\bigotimes_{j=1}^n\limits}}
\def\tprodmim{{\textstyle\bigotimes_{i=1}^m\limits}}
\def\tprodmjm{{\textstyle\bigotimes_{j=1}^m\limits}}
\def\half{{\frac12}}
\def\thalf{{\textstyle\half}}
\def\tkwart{{\textstyle{\frac14}}}
\def\tint{{\textstyle\int\limits}}
\def\tbigcap{{\textstyle\bigcap\limits}}
\def\tbigcup{{\textstyle\bigcup\limits}}
\def\ra{\rightarrow}
\def\da{\downarrow}
\def\ua{\uparrow}
\def\dotfil{\leaders\hbox to 1em{\hss.\hss}\hfill}
\def\minqquad{\hskip-2em\relax}\def\minqqqquad{\hskip-4em\relax}
\def\qqqquad{\hskip4em\relax}\def\qqqqqquad{\hskip6em\relax}
\def\liminfsup{\mathop{\overline{\underline{\rm lim}}}}





% Mathematics
\def\hexnumber#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or A\or B\or C\or D\or E\or F\fi}
%\mathchardef\boxminus="3\hexnumber\msafam0C
%\mathchardef\lesssim="3\hexnumber\msafam2E
%\mathchardef\gtrsim="3\hexnumber\msafam26
%\mathchardef\rightsquigarrow="3\hexnumber\msafam20
\def\mypartial#1{\mathchoice{\partial\over\partial#1}{\partial/\partial#1}{}{}}
\def\Re{\mathop{\rm Re}\nolimits}
\def\Im{\mathop{\rm Im}\nolimits}
\def\entier#1{\lfloor#1\rfloor}
\def\BL{{\rm B\kern -0.5pt L}}
\def\UC{{\rm U\kern-0.5pt C}}
\def\linfty{\ell^\infty}
\def\simplex{{\rm S}}
\def\id{id}
\def\argmax{\mathop{\rm argmax}}
\def\argmin{\mathop{\rm argmin}}
\def\trace{{\rm trace }}
\def\diag{\mathop{\rm diag\,}\nolimits}
\def\lin{\mathop{\rm lin\,}\nolimits}
\def\closedlin{\overline{\lin}}
\def\tanh{\mathop{\rm tanh}\nolimits}
\def\arctanh{\mathop{\rm arctanh}\nolimits}
\def\arctg{\mathop{\rm arctg}\nolimits}
\def\loglog{\mathop{\rm loglog}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
%\def\interior{{\rm int}}
\def\interior{\mathaccent 23}
\def\closure#1{\overline{#1}}
\def\boundary{\mathop{\delta}\nolimits}
\def\closedhull{{\overline{\hull}}}
\def\closedconv{\closedhull}
\def\essinf{\mathop{\rm essinf}\limits}
\def\conv{\hull}
\def\hull{\mathop{\rm conv\ }\nolimits}
\def\diam{\mathop{\rm diam}\nolimits}
\def\ball{\mathop{\rm ball}\nolimits}
\def\closedball{\overline{\ball}}
\def\every{\hbox{ every }}
\def\forevery{\hbox{ for every }}
\def\OR{\hbox{ or }}
\def\implies{\hbox{ $\Rightarrow$ }}
\def\seilpmi{\hbox{ $\Leftarrow$ }}
\def\bydef{\buildrel {\rm def}\over =}
\def\qed{\ \vrule height4pt width4pt depth0pt}
\def\halmos{\ \vbox{\hrule\hbox{\vrule\vbox{\phantom{\vrule height4pt width4pt depth0pt}}\vrule}\hrule}}

% Statistics
\def\Prodint{\mathop{\mathchoice{\vcenter{\epsfysize=1.5em\epsfbox{%
  prodint.eps}}}{\vcenter{\epsfysize=1em\epsfbox{prodint.eps}}}{}{}}}
\def\prodint{\Prodint}
\def\tdot#1{\kern1.2pt\dot{\vphantom{#1}}\kern-1.2pt
        \dot#1\kern0.8pt\dot{\vphantom{#1}}\kern-0.8pt}
\def\contiguous{\triangleleft}
\def\doublecontiguous{\mathrel{\triangleleft\,\joinrel\triangleright}}
\def\E{\mathord{\rm E}}
\def\Pr{\mathord{\rm P}}
\def\var{\mathop{\rm var}\nolimits}
\def\sdev{\mathop{\rm sd}\nolimits}
\def\cov{\mathop{\rm cov}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\cor{\mathop{\rm cor}\nolimits}
\def\Cor{\mathop{\rm Cor}\nolimits}
\let\covar\cov
\let\Covar\Cov
\let\Var=\var
\def\med{\mathop{\rm med}\nolimits}
\def\medlimits{\mathop{\rm med}\limits}
\def\almostsurely{{\rm a.s.}}
\def\almosteverywhere{{\rm a.e.}}
\def\infinitelyoften{{\rm i.o.}}
\def\ae{\almosteverywhere}
\def\ldot{\hbox {$\dot \ell$}}
\def\ltil{\hbox{$\tilde \ell$}}
\def\dirac{\delta}
\def\haslaw{\sim}
\def\haslawunder#1{\mathchoice{\buildrel #1\over \sim}{\ \mathrel{^{#1}}\joinrel\sim}{}{}}
\def\generatedby{\s}
\mathchardef\given="626A
\mathcode`:="603A
%\mathchardef\setminus="2200


% Convergence symbols
\def\generalweak#1{\ {\mathchoice{\buildrel #1\over \rightsquigarrow}%
{\raise-2pt\hbox{$\buildrel #1\over \rightsquigarrow$}}{}{}}\ }
\let\weak\rightsquigarrow
\def\generalprob#1{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel#1\over\ra$}}
{\raise-2pt\hbox{$\buildrel#1\over\ra$}}{}{}}\ }
\def\outerp{\generalprob {\small P*}}
\def\prob{\generalprob{\small P}}
\def\outeras{\generalprob{\small as*}}
\def\as{\generalprob{\small as}}
\def\vague{\generalprob{\small v}}
\def\au{\generalprob{\small au}}
\def\Pgg{\ {\mathchoice{\raise-1.5pt\hbox{$\buildrel {\small P}\over\gg$}}
{\raise-2pt\hbox{$\buildrel {\small P}\over\gg$}}{}{}}\ }

% Miscellaneous
\def\beginskip{\begingroup\long\def\eet##1\endskip{\endgroup}\eet}
\def\endskip{}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern1pt\vbox{\kern1pt #1\kern1pt}\kern1pt\vrule}\hrule}}
\def\eet#1{}
\def\makenumbersactive{\catcode`\0=11\catcode`\1=11\catcode`\2=11%
        \catcode`\3=11\catcode`\4=11\catcode`\5=11%
        \catcode`\6=11\catcode`\7=11\catcode`\8=11\catcode`\9=11 }



\catcode`\@=12







